Stochastic Processes in Mesoscale Physics and the Early Universe

This thesis is dedicated to the study of stochastic processes; non-deterministic physical phenomena that can be well described by classical physics. The stochastic processes we are interested in are akin to Brownian Motion and can be described by an overdamped Langevin equation comprised of a deterministic drift term and a random noise term. In Part I we examine stochastic processes in the Mesoscale. For us this means that the Langevin equation is driven by thermal noise, with amplitude proportional to the temperature $T$ and there exists a genuine equilibrium thermal state. We apply a technique known as the Functional Renormalisation Group (FRG) which allows us to coarse-grain in temporal scales. We describe how to obtain effective equations of motion for the 1- and 2-point functions of a particle evolving in highly non-trivial potentials and verify their accuracy by comparison to direct numerical simulations. In this way we outline a novel procedure for describing the behaviour of stochastic processes without having to resort to time consuming numerical simulations. In Part II we turn to the Early Universe and in particular examine stochastic processes occurring during a period of accelerated expansion known as inflation. This inflationary period is driven by a scalar field called the inflaton which also obeys a Langevin equation in the Stochastic Inflation formalism. We use this to study the formation of Primordial Black Holes during a period of Ultra Slow-Roll. We finish this thesis by applying the techniques developed in Part I to a spectator field during inflation. FRG techniques can compute cosmologically relevant observables such as the power spectrum and spectral tilt. We also extend the FRG formalism to solve first-passage time problems and verify that it gives the correct prediction for the average time taken for a field (or particle) to overcome a barrier in the potential.

==> Chapters/Chapter01.tex <==
% Chapter 1

\chapter{Introduction} % Chapter title

\label{ch:introduction} % For referencing the chapter elsewhere, use \autoref{ch:introduction} 

%----------------------------------------------------------------------------------------

This template for \LaTeX\ has two goals:
\begin{enumerate}
\item Provide students with an easy-to-use template for their Master's or PhD thesis (though it might also be used by other types of authors for reports, books, etc.).
\item Provide a classic, high-quality typographic style that is inspired by \citeauthor{bringhurst:2002}'s ``\emph{The Elements of Typographic Style}'' \citep{bringhurst:2002}.
\marginpar{\myTitle \myVersion}
\end{enumerate}

The bundle is configured to run with a \emph{full} MiK\TeX\ or \TeX Live installation right away and, therefore, it uses only freely available fonts.

People interested only in the nice style and not the whole bundle can now use the style stand-alone via the file \texttt{classicthesis.sty}. This works now also with ``plain'' \LaTeX.

As of version 3.0, \texttt{classicthesis} can also be easily used with \mLyX\footnote{\url{http://www.lyx.org}} thanks to Nicholas Mariette and Ivo Pletikosi\'c. The \mLyX\ version of this manual will contain more information on the details.

This should enable anyone with a basic knowledge of \LaTeXe\ or \mLyX\ to produce beautiful documents without too much effort. In the end, this is my overall goal: more beautiful documents, especially theses, as I am tired of seeing so many ugly ones.

The whole template and the used style is released under the \textsmaller{GNU} General Public License. 

If you like the style then I would appreciate a postcard:
\begin{center}
André Miede \\
Detmolder Straße 32 \\
31737 Rinteln \\
Germany
\end{center}

\noindent The postcards I received so far are available at:
\begin{center}
 \url{http://postcards.miede.de}
\end{center}
\marginpar{A well-balanced line width improves the legibility of the text. That's what typography is all about, right?} So far, many theses, some books, and several other publications have been typeset successfully with it. If you are interested in some typographic details behind it, enjoy Robert Bringhurst's wonderful book. % \citep{bringhurst:2002}.

\paragraph{Important Note:} Some things of this style might look unusual at first glance, many people feel so in the beginning. However, all things are intentionally designed to be as they are, especially these:
\begin{itemize}
\item No bold fonts are used. Italics or spaced small caps do the job quite well.
\item The size of the text body is intentionally shaped like it is. It supports both legibility and allows a reasonable amount of information to be on a page. And, no: the lines are not too short.
\item The tables intentionally do not use vertical or double rules. See the documentation for the \texttt{booktabs} package for a nice discussion of this topic.\footnote{To be found online at \\ \url{http://www.ctan.org/tex-archive/macros/latex/contrib/booktabs/}.}
\item And last but not least, to provide the reader with a way easier access to page numbers in the table of contents, the page numbers are right behind the titles. Yes, they are \emph{not} neatly aligned at the right side and they are \emph{not} connected with dots that help the eye to bridge a distance that is not necessary. If you are still not convinced: is your reader interested in the page number or does she want to sum the numbers up?
\end{itemize}

\noindent Therefore, please do not break the beauty of the style by changing these things unless you really know what you are doing! Please.

\paragraph{Yet Another Important Note:} Since \texttt{classicthesis}' first release in 2006, many things have changed in the \LaTeX\ world.  Trying to keep up-to-date, \texttt{classicthesis} grew and evolved into many directions, trying to stay (some kind of) stable and be compatible with its port to \mLyX. However, there are still many remains from older times in the code, many dirty workarounds here and there, and several other things I am absolutely not proud of (for example my unwise combination of \acsfont{KOMA} and \texttt{titlesec} etc.). \graffito{An outlook into the future of \texttt{classicthesis}.}

Currently, I am looking into how to completely re-design and re-implement \texttt{classicthesis} making it easier to maintain and to use. As a general idea, \texttt{classicthesis.sty} should be developed and distributed separately from the template bundle itself. Excellent spin-offs such as \texttt{arsclassica} could also be integrated (with permission by their authors) as format configurations. Also, current trends of \texttt{microtype}, \texttt{fontspec}, etc. should be included as well. As I am not really into deep \LaTeX\ programming, I will reach out to the \LaTeX\ community for their expertise and help.

%----------------------------------------------------------------------------------------

\section{Organization}
A very important factor for successful thesis writing is the organization of the material. This template suggests a structure as the following:
\begin{itemize}
\marginpar{You can use these margins for summaries of the text body\dots}
\item\texttt{Chapters/} is where all the ``real'' content goes in separate files such as \texttt{Chapter01.tex} etc.
\item\texttt{FrontBackMatter/} is where all the stuff goes that surrounds the ``real'' content, such as the acknowledgments, dedication, etc.
\item\texttt{gfx/} is where you put all the graphics you use in the thesis. Maybe they should be organized into subfolders depending on the chapter they are used in, if you have a lot of graphics.
\item\texttt{Bibliography.bib}: the Bib\TeX\ database to organize all the references you might want to cite.
\item\texttt{classicthesis.sty}: the style definition to get this awesome look and feel. Bonus: works with both \LaTeX\ and \textsc{pdf}\LaTeX\dots and \mLyX.
\item\texttt{ClassicThesis.tcp} a \TeX nicCenter project file. Great tool and it's free!
\item\texttt{ClassicThesis.tex}: the main file of your thesis where all the content gets bundled together.
\item\texttt{classicthesis-config.tex}: a central place to load all nifty packages that are used. In there, you can also activate backrefs in order to have information in the bibliography about where a source was cited in the text (\ie, the page number).
    
\emph{Make your changes and adjustments here.} This means that you specify here the options you want to load \texttt{classicthesis.sty} with. You also adjust the title of your thesis, your name, and all similar information here. Refer to \autoref{sec:custom} for more information.

This had to change as of version 3.0 in order to enable an easy transition from the ``basic'' style to \mLyX.
\end{itemize}

\noindent In total, this should get you started in no time.

%----------------------------------------------------------------------------------------

\section{Style Options}\label{sec:options}

There are a couple of options for \texttt{classicthesis.sty} that allow for a bit of freedom concerning the layout: \marginpar{\dots or your supervisor might use the margins for some comments of her own while reading.}
\begin{itemize}
\item General:
\begin{itemize}
\item\texttt{drafting}: prints the date and time at the bottom of each page, so you always know which version you are dealing with. Might come in handy not to give your Prof. that old draft.
\end{itemize}
	
\item Parts and Chapters:
\begin{itemize}
\item\texttt{parts}: if you use Part divisions for your document, you should choose this option. (Cannot be used together with \texttt{nochapters}.)

\item\texttt{nochapters}: allows to use the look-and-feel with classes that do not use chapters, \eg, for articles. Automatically turns off a couple of other options: \texttt{eulerchapternumbers}, \texttt{linedheaders}, \texttt{listsseparated}, and \texttt{parts}. 

\item\texttt{linedheaders}: changes the look of the chapter headings a bit by adding a horizontal line above the chapter title. The chapter number will also be moved to the top of the page, above the chapter title.
\end{itemize}

\item Typography:
\begin{itemize}
\item\texttt{eulerchapternumbers}: use figures from Hermann Zapf's Euler math font for the chapter numbers. By default, old style figures from the Palatino font are used.

\item\texttt{beramono}: loads Bera Mono as typewriter font. (Default setting is using the standard CM typewriter font.)

\item\texttt{eulermath}: loads the awesome Euler fonts for math. (Palatino is used as default font.)

\item\texttt{pdfspacing}: makes use of pdftex' letter spacing capabilities via the \texttt{microtype} package.\footnote{Use \texttt{microtype}'s \texttt{DVIoutput} option to generate DVI with pdftex.} This fixes some serious issues regarding math formul\ae\ etc. (\eg, ``\ss'') in headers. 

\item\texttt{minionprospacing}: uses the internal \texttt{textssc} command of the \texttt{MinionPro} package for letter spacing. This automatically enables the \texttt{minionpro} option and overrides the \texttt{pdfspacing} option.
\end{itemize}  

\item Table of Contents:
\begin{itemize}
\item\texttt{tocaligned}: aligns the whole table of contents on the left side. Some people like that, some don't.

\item\texttt{dottedtoc}: sets pagenumbers flushed right in the table of contents.

\item\texttt{manychapters}: if you need more than nine chapters for your document, you might not be happy with the spacing between the chapter number and the chapter title in the Table of Contents. This option allows for additional space in this context. However, it does not look as ``perfect'' if you use \verb|\parts| for structuring your document.
\end{itemize}

\item Floats:
\begin{itemize}
\item\texttt{listings}: loads the \texttt{listings} package (if not already done) and configures the List of Listings accordingly.
    
\item\texttt{floatperchapter}: activates numbering per chapter for all floats such as figures, tables, and listings (if used).	
    
\item\texttt{subfig}(\texttt{ure}): is passed to the \texttt{tocloft} package to enable compatibility with the \texttt{subfig}(\texttt{ure}) package. Use this option if you want use classicthesis with the \texttt{subfig} package.

\end{itemize}    

\end{itemize}

\noindent The best way to figure these options out is to try the different possibilities and see, what you and your supervisor like best.

In order to make things easier in general, \texttt{classicthesis-config.tex} contains some useful commands that might help you.

%----------------------------------------------------------------------------------------

\section{Customization}\label{sec:custom}

This section will give you some hints about how to adapt \texttt{classicthesis} to your needs.

The file \texttt{classicthesis.sty} contains the core functionality of the style and in most cases will be left intact, whereas the file \texttt{classic\-thesis-config.tex} is used for some common user customizations. 

The first customization you are about to make is to alter the document title, author name, and other thesis details. In order to do this, replace the data in the following lines of \texttt{classicthesis-config.tex:}\marginpar{Modifications in \texttt{classic\-thesis-config.tex}
}

\begin{lstlisting}
\newcommand{\myTitle}{A Classic Thesis Style\xspace}
\newcommand{\mySubtitle}{An Homage to ...\xspace}
\end{lstlisting}

Further customization can be made in \texttt{classicthesis-config.tex} by choosing the options to \texttt{classicthesis.sty} (see~\autoref{sec:options}) in a line that looks like this:

\begin{lstlisting}
\PassOptionsToPackage{eulerchapternumbers,listings,drafting, pdfspacing, subfig,beramono,eulermath,parts}{classicthesis}
\end{lstlisting}

Many other customizations in \texttt{classicthesis-config.tex} are possible, but you should be careful making changes there, since some changes could cause errors.

Finally, changes can be made in the file \texttt{classicthesis.sty}, \marginpar{Modifications in \texttt{classicthesis.sty}} although this is mostly not designed for user customization. The main change that might be made here is the text-block size, for example, to get longer lines of text.

%----------------------------------------------------------------------------------------

\section{Issues}\label{sec:issues}
This section will list some information about problems using \texttt{classic\-thesis} in general or using it with other packages.

Beta versions of \texttt{classicthesis} can be found at Bitbucket:
\begin{center}
    \url{https://bitbucket.org/amiede/classicthesis/}
\end{center}
There, you can also post serious bugs and problems you encounter.

\subsection*{Compatibility with the \texttt{glossaries} Package}
If you want to use the \texttt{glossaries} package, take care of loading it with the following options:
\begin{verbatim}
\usepackage[style=long,nolist]{glossaries}
\end{verbatim}

\noindent Thanks to Sven Staehs for this information. 

\subsection*{Compatibility with the (Spanish) \texttt{babel} Package}
Spanish languages need an extra option in order to work with this template:
\begin{lstlisting}
    \usepackage[spanish,es-lcroman]{babel}
\end{lstlisting}
Thanks to an unknown person for this information (via the issue reporting). 

\paragraph{Further information for using \texttt{classicthesis} with Spanish (in addition to the above)}
In the file \texttt{ClassicThesis.tex} activate the language: 
\begin{lstlisting}
    \selectlanguage{spanish}
\end{lstlisting}

If there are issues changing \verb|\tablename|, \eg, using this:
\begin{lstlisting}
    \renewcommand{\tablename}{Tabla}
\end{lstlisting}

This can be solved by passing \texttt{es-tabla} parameter to \texttt{babel}:
\begin{lstlisting}
    \PassOptionsToPackage{es-tabla,spanish,es-lcroman,english}{babel}
    \usepackage{babel}
\end{lstlisting}

But it is also necessary to set \texttt{spanish} in the \verb|\documentclass|.

Thanks to Alvaro Jaramillo Duque for this information. 

\subsection*{Compatibility with the \texttt{pdfsync} Package}
Using the \texttt{pdfsync} package leads to linebreaking problems with the \texttt{graffito} command. Thanks to Henrik Schumacher for this information. 

%----------------------------------------------------------------------------------------

\section{Future Work}
So far, this is a quite stable version that served a couple of people well during their thesis time. However, some things are still not as they should be. Proper documentation in the standard format is still missing. In the long run, the style should probably be published separately, with the template bundle being only an application of the style. Alas, there is no time for that at the moment\dots it could be a nice task for a small group of \LaTeX nicians.

Please do not send me email with questions concerning \LaTeX\ or the template, as I do not have time for an answer. But if you have comments, suggestions, or improvements for the style or the template in general, do not hesitate to write them on that postcard of yours.

%----------------------------------------------------------------------------------------

\section{Beyond a Thesis}
The layout of \texttt{classicthesis.sty} can be easily used without the framework of this template. A few examples where it was used to typeset an article, a book or a curriculum vitae can be found in the folder \texttt{Examples}. The examples have been tested with \texttt{latex} and \texttt{pdflatex} and are easy to compile. To encourage you even more, PDFs built from the sources can be found in the same folder.

%----------------------------------------------------------------------------------------

\section{License}
\paragraph{GNU General Public License:} This program is free software; you can redistribute it and/or modify it under the terms of the \textsmaller{GNU} General Public License as published by the Free Software Foundation; either version 2 of the License, or (at your option) any later version.

This program is distributed in the hope that it will be useful, but \emph{without any warranty}; without even the implied warranty of \emph{merchantability} or \emph{fitness for a particular purpose}. See the \textsmaller{GNU} General Public License for more details.

==> Chapters/Chapter04.tex <==
% Chapter X

\chapter{Chapter Title} % Chapter title

\label{ch:name} % For referencing the chapter elsewhere, use \autoref{ch:name} 

%----------------------------------------------------------------------------------------

\section{Section Title}

Content

%------------------------------------------------

\subsection{Subsection Title}

Content

%------------------------------------------------

\subsection{Subsection Title}

Content

%----------------------------------------------------------------------------------------

\section{Section Title}

Content

==> Chapters/Chapter0B.tex <==
% Appendix X

\chapter{Appendix Title}

%----------------------------------------------------------------------------------------

% Content begins here

==> FrontBackMatter/Colophon.tex <==
% Colophon (a brief description of publication or production notes relevant to the edition)

\pagestyle{empty}

\hfill

\vfill

\pdfbookmark[0]{Colophon}{colophon}

\section*{Colophon}

This document was typeset using the typographical look-and-feel \texttt{classicthesis} developed by Andr\'e Miede. The style was inspired by Robert Bringhurst's seminal book on typography ``\emph{The Elements of Typographic Style}''. \texttt{classicthesis} is available for both \LaTeX\ and \mLyX: 

\begin{center}
\url{https://bitbucket.org/amiede/classicthesis/}
\end{center}

\noindent Happy users of \texttt{classicthesis} usually send a real postcard to the author, a collection of postcards received so far is featured here: 

\begin{center}
\url{http://postcards.miede.de/}
\end{center}
 
\bigskip

\noindent\finalVersionString

==> FrontBackMatter/Publications.tex <==
% Publications - a page listing research articles written using content in the thesis

\pdfbookmark[1]{Publications}{Publications} % Bookmark name visible in a PDF viewer

\chapter*{Publications} % Publications page text

Some ideas and figures have appeared previously in the following publications:\\

\cite{Wilkins2020a}\cite{Rigopoulos2021}
%\begin{refsection}[ownpubs]
%    \small
%    \nocite{*} % is local to to the enclosing refsection
%    \printbibliography[heading=none]
%\end{refsection}

%\emph{Attention}: This requires a separate run of \texttt{bibtex} for your \texttt{refsection}, \eg, \texttt{ClassicThesis1-blx} for this file. You might also use \texttt{biber} as the backend for \texttt{biblatex}. See also \url{http://tex.stackexchange.com/questions/128196/problem-with-refsection}.
